ABPT: Amended Backpropagation through Time with Partially Differentiable Rewards

Quadrotor control policies can be trained with high performance using the exact gradients of the rewards to directly optimize policy parameters via backpropagation-through-time (BPTT). However, designing a fully differentiable reward architecture is often challenging. Partially differentiable rewards will result in biased gradient propagation that degrades training performance. To overcome this limitation, we propose Amended Backpropagation-through-Time (ABPT), a novel approach that mitigates gradient bias while preserving the training efficiency of BPTT. ABPT combines 0-step and N-step returns, effectively reducing the bias by leveraging value gradients from the learned Q-value function. Additionally, it adopts entropy regularization and state initialization mechanisms to encourage exploration during training. We evaluate ABPT on four representative quadrotor flight tasks \li{in both real world and simulation}. Experimental results demonstrate that ABPT converges significantly faster and achieves higher ultimate rewards than existing learning algorithms, particularly in tasks involving partially differentiable rewards. The code will be released at http://github.com/Fanxing-LI/ABPT.

==> realWorldExperiment.tex <==
\label{sec:realWorldExp}
% \li{
% %围绕主题讲，不要偏题
% Excluding algorithm validation, our sim-to-real and sim-to-sim (to AirSim) experiments reveal that aggressive policies, such as racing, show a much smaller performance gap across different physical environments compared to gentle policies like hovering—regardless of variations in communication delay, control output response, or drone weight characteristics.
% This difference arises because aggressive policies have a non-zero expected average output over short time horizons, meaning the action sign becomes more robust. In contrast, gentle policies, which typically have near-zero expected output, are more sensitive to environmental discrepancies, making them prone to instability or even inversion under varying conditions. From another perspective, although it seems that high-speed flight is much difficult compared to hovering, in fact hovering is sometimes harder and the most appropriate benchmark to validate whether the gap is well eliminated.
\zou{We have validate our trained policies in real-world experiments. Some results are shown in ~\reffig{fig:real_world_hover} and ~\reffig{fig:real_world_landing}. More results are demonstrated in the supplementary video.}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/real_world.png}
    \caption{\textbf{Hover}: our trained policy leads to more stable trajectories compared to the policy trained by PPO.}
    \label{fig:real_world_hover}
\end{figure*}

